Two-Stage Constrained Actor-Critic for Short Video Recommendation

The wide popularity of short videos on social media poses new opportunities and challenges to optimize recommender systems on the video-sharing platforms. Users sequentially interact with the system and provide complex and multi-faceted responses, including watch time and various types of interactions with multiple videos. One the one hand, the platforms aims at optimizing the users' cumulative watch time (main goal) in long term, which can be effectively optimized by Reinforcement Learning. On the other hand, the platforms also needs to satisfy the constraint of accommodating the responses of multiple user interactions (auxiliary goals) such like, follow, share etc. In this paper, we formulate the problem of short video recommendation as a Constrained Markov Decision Process (CMDP). We find that traditional constrained reinforcement learning algorithms can not work well in this setting. We propose a novel two-stage constrained actor-critic method: At stage one, we learn individual policies to optimize each auxiliary signal. At stage two, we learn a policy to (i) optimize the main signal and (ii) stay close to policies learned at the first stage, which effectively guarantees the performance of this main policy on the auxiliaries. Through extensive offline evaluations, we demonstrate effectiveness of our method over alternatives in both optimizing the main goal as well as balancing the others. We further show the advantage of our method in live experiments of short video recommendations, where it significantly outperforms other baselines in terms of both watch time and interactions. Our approach has been fully launched in the production system to optimize user experiences on the platform.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> tripadvisor_backup.tex <==
\section{Offline Experiments}
\label{sec:offline}
%~\footnote{Reproduction code is released at \url{https://github.com/KuaiReco/ks-constrained-rl-rs}}
In this section, we evaluate our approach on a public dataset via extensive offline learning simulations. We demonstrate the effectiveness of our approach as compared to existing baselines in both achieving the main goal and balancing the auxiliaries. 


\iffalse
\begin{table*}[]
    \centering
    \begin{tabular}{ccccccccc}
    \toprule
        Algorithms &  service & business & cleanliness & check-in & value & rooms & location & overall \\
        \midrule
 BC & 3.38 & -1.86 & 3.57 & -0.73 & 3.32 & 2.92 & 2.93 & 3.92\\
 \midrule
 Wide\&Deep &  3.41 (0.03) & -1.86 (0.0) & 3.62 (0.05) & -0.75 (-0.02) & 3.36 (0.04) & 2.96 (0.04) & 2.88 (-0.05) & 3.98 (0.06)\\
 \midrule
 DeepFM & \textbf{3.43 (0.05)}  & -1.83 (0.03) & \textbf{3.64 (0.07)} & -0.75 (-0.02) & \textbf{3.37 (0.05)} & 2.97 (0.05) & 2.91 (-0.02) & \textbf{3.99 (0.07)}\\
  \midrule
 A3C & 3.37 (-0.01) & \textbf{-1.78 (0.08)} & 3.56 (-0.01) & -0.65 (0.08) & 3.27 (-0.05) & 2.95 (0.03) & 2.88 (-0.05)& 3.94 (0.02)\\
 \midrule
 DDPG & 3.40 (0.02) & -1.82 (0.04) & 3.61 (0.04) & -0.71 (0.02) & 3.34 (0.02) & 2.95 (0.03) & 2.91 (-0.02) & 3.97 (0.05)\\
\midrule
RCPO-DDPG & 
3.41 (0.03) & -1.82 (0.04) & 3.62 (0.05) & -0.68 (0.05) & 3.35 (0.03) & 2.97 (0.04)&2.87 (-0.06) & \textbf{3.99 (0.07)}\\
\midrule
 Pareto-DDPG & 3.36 (-0.02) & -1.79 (0.07) &3.57 (0.0) & \textbf{-0.62 (0.11)} & 3.29 (-0.03) & 2.93 (0.01) & 2.86 (-0.07)  & 3.95 (0.03)\\
 \midrule
Constrained-DDPG (Ours) & \textbf{3.43 (0.05)} & -1.82 (0.04) & \textbf{3.64 (0.07)}& -0.68 (0.05) & \textbf{3.37 (0.05)} & \textbf{3.00 (0.08)} & \textbf{2.98 (0.05)} & \textbf{3.99 (0.07)}\\
\bottomrule
    \end{tabular}
    \caption{Performance of different algorithms on an offline dataset.}
    \label{tab:offline}
\end{table*}
\fi




\subsection{Setup}
\paragraph{Dataset} We consider a  hotel-review dataset named \emph{TripAdvisor}, which is a standard dataset for studying policy optimization in recommender system with multiple responses in \cite{chen2021reinforcement}. 
In this data, customers not only provide an \emph{overall} rating for hotels but also score hotels in multiple aspects including \emph{service}, \emph{business}, \emph{cleanliness}, \emph{check-in}, \emph{value}, \emph{rooms}, and \emph{location} \cite{alam2016joint}.
\footnote{The dataset consists of both the main objective and other responses, which can also be used to evaluate constrained policy optimization in recommender system.} Reviews provided by the same user are concatenated chronologically to form a trajectory; we filter trajectories with length smaller than $20$.
In total, we have $20277$ customers, $150$ hotels, and $257932$ reviews. 

\paragraph{MDP} A trajectory tracks a customer hotel-reviewing history.  For each  review, we have
\iffalse
\begin{itemize}
    \item state $s_t$: customer ID and  the last three reviewed hotel IDs as well as corresponding multi-aspect review scores.
    \item action $a_t$: currently reviewed hotel ID.
    \item reward $r_t$: a vector of eight scores the customer provided for the reviewed hotel in terms of \emph{service}, \emph{business}, \emph{cleanliness}, \emph{check-in}, \emph{value}, \emph{rooms},  \emph{location}, and \emph{overall}. 
\end{itemize}
\fi
state $s_t$: customer ID and  the last three reviewed hotel IDs as well as corresponding multi-aspect review scores; action $a_t$: currently reviewed hotel ID; reward $r_t$: a vector of eight scores the customer provided for the reviewed hotel in terms of \emph{service}, \emph{business}, \emph{cleanliness}, \emph{check-in}, \emph{value}, \emph{rooms},  \emph{location}, and \emph{overall rating}; discount factor $\gamma$: 0.99. We set the main goal to be maximizing the cumulative overall rating, and treat others as the auxiliaries. 

%\subsubsection{Evaluation Method and Hyper-parameters}
\paragraph{Evaluation}  We use the \emph{Normalised Capped Importance Sampling} ((NCIS) approach to evaluate different policies, which is a standard offline evaluation method in literature \cite{swaminathan2015self}. 
%For the 
%Lagrangian multiplier, we choose the optimal value. %We further conduct ablation studies to understand how different factors would affect our algorithm’s performance(due to lack of space, please refer to Appendix E).


\paragraph{Compared algorithms}\label{sec:alg} We compare our approach with a range of recommendation algorithms.
\begin{itemize}
    \item \textbf{BC}: a supervised behavior-cloning policy $\pi_\beta$ to mimic customer reviewing pattern, with input as the user state and output as the reviewed hotel ID. 
    \item \textbf{Wide\&Deep}\cite{cheng2016wide}: a supervised model which utilizes wide and deep layers to balance both memorization and generalization, with  input as the user state, output as the reviewed hotel id, and sample weight as the weighted sum of $8$ scores for this review. 
    %\item \textbf{DeepFM\cite{guo2017deepfm}}: a supervised recommendation model which combines deep neural network and factorization machine, with input as the user state, output as the reviewed hotel id, and sample weight as the weighted sum of $8$ scores for this review.
    \item \textbf{A3C}\cite{mnih2016asynchronous}: an online RL approach with one actor and one critic, where reward  is the  weighted sum of $8$ scores for a given customer-hotel review.
    \item \textbf{DDPG}\cite{lillicrap2015continuous}: an offline RL approach with one actor and one critic, where reward is the  weighted sum of $8$ scores for a given customer-hotel review. 
    \item \textbf{RCPO}: an offline RL approach that extends the reward-constrained policy optimization of A3C algorithm in \cite{tessler2018reward} to DDPG algorithm. 
    %Contrary to the standard DDPG, we learn eight critics for the eight scores and use Lagrangian multipliers to sum them up for the actor optimization.  
    \item \textbf{Pareto}: a recommendation model based on DDPG algorithm to find the Pareto optimal solution for multi-objective optimization.
    \item \textbf{TSCAC}: our proposed two-stage constrained actor critic algorithm, where the construction follows the discussion in Section \ref{sec:ddpg}. 
\end{itemize}
 We note that we use DDPG instead of A3C as the base actor critic model to develop constrained policy optimization (RCPO, Pareto, and TSCAC), by the nature of offline learning. As a comparison, we also present the performance of A3C, which is for online learning and thus is outperformed by DDPG on this dataset---as we shall see shortly. 

%\subsubsection{Evaluation Metric}
%We use the \emph{Normalised Capped Importance Sampling} ((NCIS) approach to evaluate different policies, which is a standard offline evaluation method in literature \cite{swaminathan2015self}. 
\iffalse
Specifically, denote $\pi_\beta$ as the behavior policy of the dataset, denote $\pi$ as the learned policy, we evaluate it on the dataset as follows: 
$
    \hat{V}^{NCIS}(\pi) & = \frac{\sum_{(s,a,r)} \bar{w}_{\pi,\pi_\beta}(s,a) r }{\sum_{(s,a,r)} \bar{w}_{\pi,\pi_\beta}(s,a)},
    \mbox{where}\quad & \bar{w}_{\pi,\pi_\beta}(s,a) =\mbox{clip}\bigg( \frac{\phi_{\pi(s)}(a) }{\phi_{\pi_\beta(s)}(a)}, c\bigg).
$
 Here $\phi_{\pi(s)}$ and $\phi_{\pi_\beta(s)}$ are probability density functions of normal distributions with means $\pi(s)$ and $\pi_\beta(s)$ respectively.
\fi
\subsection{Overall Performance}


\begin{table*}
    \centering
     \renewcommand\arraystretch{1.5} 
    \begin{tabular}{c|ccc cccc|c}
    \hline
        Algorithm &  BC &  Wide\&Deep & A3C & DDPG & RCPO & Pareto & TSCAC  \\
  \hline
  Service	&	$3.38$	& 	$3.41^{*}$	&		$3.37$	&	$3.4$	&	$3.41$	&	$3.36$	& $\mathbf{3.43}$ \\  
  \hline
  Business	&	$-1.86$	& 	$-1.86$	& $-1.78^{*}$	&	$-1.82$	&	$-1.82$	&	$-1.79$	&	-1.82		\\
  \hline
  Cleanliness	&	$3.57$	& 	$3.62^{*}$	&		$3.56$	&	$3.61$	&	$3.62^{*}$	&	3.57	&	$\mathbf{3.64}$		\\
  \hline
  Check-in	&	$-0.73$	& 	$-0.75$	&		$-0.65$	&	$-0.71$	&	$-0.68$	&	$-0.62^{*}$	&	$-0.68$		\\
  \hline
  Value	&	$3.32$	& 	$3.36^{*}$	&		$3.27$	&	$3.34$	&	$3.35$	&	$3.29$	&	$\mathbf{3.37}$		\\
  \hline
  Rooms	&	$2.92$	& 	$2.96$	&	$2.97^{*}$		&	$2.95$	&	$2.97^{*}$	&	$2.93$	&	\textbf{3.00}		\\ \hline
  Location	&	$2.93^{*}$	& 	$2.88$	& 	$2.88$	&	$2.91$	&	$2.87$	&	$2.86$	&	\textbf{2.98}		\\ \hline
  Overall Rating	&	$3.92$	& 	$3.98$		& 	$3.94$	&	$3.97$	&	$\mathbf{3.99}^{*}$	&	$3.95$	&	 $\mathbf{3.99}$		\\ \hline
  
%\bottomrule
    \end{tabular}
\caption{Performance of different algorithms on an offline dataset. The results with $*$ denote the best performance among all baseline methods in each response dimension, and the data in last column is marked by bold font when our constrained-DDPG achieves the best performance. }
\label{tab:offlineV2}
\end{table*}

Table \ref{tab:offlineV2} presents the results of different algorithms in terms of eight scores. First note that A3C is outperformed by DDPG in most scores, which is as expected since A3C is an online learning algorithm that does not fit the offline setup here; this justifies our comparison focusing on DDPG-based constrained RL algorithms.  We can see that our  approach Constrained-DDPG performs the best among all algorithms: for the main goal, Constrained-DDPG achieves the highest overall rating $3.99$; for the auxiliary goal,  Constrained-DDPG also ranks highest for $5$ out of $7$  scores (service, cleanliness, value, rooms, location). The Pareto algorithm indeed learns a Pareto-optimal solution that achieves best performance on the check-in score, which however does not satisfy the setting here with the main goal to optimize the overall rating. The RCPO algorithm achieves the same best  overall score as our approach, but they sacrifice much on the others, and in particular, the location score is even lower than that from the BC algorithm.



\subsection{Ablation Study}
We investigate how the Lagrangian multiplier, which controls the strength of constraint, affects our model performance.  We vary $\lambda$ across $[1e-8, 2.56e-6, 1e-4, 1.6e-3, 1, 1e4]$ and present  performance of our constrained-DDPG in terms of all eight scores. Recall that larger $\lambda$ denotes stronger constraint that optimizes scores other than the overall one. Figure \ref{fig:offline-ablation} shows that with $\lambda$ increasing, our policy performance is also improved on most constraint scores (including service, business, cleanliness, value, rooms, and location), which is as expected since the learned policy becomes closer to the constraint policy that optimizes those scores. 
%We also note that overall score is not sensitive to the Lagrangian multiplier and remains around $3.986$ for various $\lambda$ values.

\begin{figure*}
    \centering
    \includegraphics[width=18cm]{ablation_v5.pdf}
    \caption{Effect of Lagrangian multiplier on model performance. The X-axis is the  of Lagrangian multiplier and the Y-axis is the score of each response.}
    \label{fig:offline-ablation}
\end{figure*}

\iffalse
\paragraph{The Effect of the discount factor on the performance} As a critical hyper-parameter in RL methods, the discount factor $\gamma$ plays a vital role in model performance. To this end, we study the influence of $\gamma$ and range its value across $[0.5, 0.7, 0.9, 0.99, 0.999]$. We present our model performance on the main response (overall score) and one auxiliary task (business score); results of other scores are shown in Appendix \ref{appendix:offline_results} to conserve space. The results are shown in Figure \ref{fig:offline-gamma} . We can see that as $\gamma$ increases, our policy progressively delivers improved performance for the main response since the long term reward is further considered, while the performance on  the auxiliary task first remains relatively stable and then peaks for $\gamma=0.99$. However, the policy performance may deteriorate when $\gamma$ is too large. In this dataset, We select $\gamma = 0.99$ as an appropriate choice. 

\begin{figure}
    \centering
    \includegraphics[width=8cm, height=4cm]{discount_factor_v5.pdf}
    \caption{Effect of Discount Factor on model performance.}
    \label{fig:offline-gamma}
\end{figure}

% \begin{table*}[]
%     \centering
%     \begin{tabular}{ccccccccc}
%     \toprule
%      $\lambda$ &  service & business & cleanliness & check-in & value & rooms & location & overall \\
%         \midrule
%         1e-8 &	3.426 &	-1.818 &	3.633 &	-0.669 &	3.367 &	2.991 &	2.969 &	3.985
% \\
%  \midrule
% 2.56e-6 &	3.425 &	-1.818 &	3.633 &	-0.669 &	3.366 &	2.991 &	2.969 &	3.984
% \\
%   \midrule
% 1e-4 &	3.430 &	-1.817 &	3.637 &	-0.676 &	3.370 &	2.997 &	2.975 &	3.987
% \\
%  \midrule
% 1.6e-3 &	3.431 &	-1.816 &	3.638 &	-0.675 &	3.371 &	2.998	 &2.976 &	3.987
% \\
%  \midrule
% 1 &	3.432 &	-1.816 &	3.639 &	-0.677 &	3.372 &	2.999 &	2.978 &	3.988
% \\
% \midrule
%  1e4 & 3.430 &	-1.815 &	3.638 &	-0.665 &	3.370 &	2.998 &	2.975 &	3.985\\
% \bottomrule
%     \end{tabular}
%     \caption{Performance of different algorithms on an offline dataset.}
%     \label{tab:offline-ablation}
% \end{table*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{ablation_v5.pdf}
    \caption{Effect of Lagrangian multiplier on model performance. The X-axis is the  of Lagrangian multiplier and the Y-axis is the score of each response.}
    \label{fig:offline-ablation}
\end{figure*}

%\subsubsection{The effect of the number of constraints on the performance}
\fi


